Immersed boundary-conformal isogeometric methods for magnetostatics

Isogeometric analysis was proposed to bridge the gap between computer-aided design and numerical discretization. However, standard multi-patch isogeometric analysis mandates conformal discretizations across patch interfaces, posing challenges for multi-material domain problems. In the context of electric machines, this requirement becomes evident in a large number of patches needed to represent machines consisting of several domains and materials. In this work, we adopt, extend, and evaluate three non-conformal discretization strategies for magnetostatic problems: a fully immersed approach, the union with non-conformal patches, and the union with conformal layers. In all three methods, boundary-conformal high-order quadrature rules are employed for integration over trimmed boundary and interface elements. In the two union approaches, material regions are, as far as possible, represented by independent non-conformal spline patches that are embedded within a background patch and coupled weakly through Nitsche's method. In the latter framework, critical interfaces are additionally surrounded by conformal layers that enable the strong imposition of boundary conditions and improved resolution of interface behavior. The proposed approaches are assessed through several magnetostatic benchmark problems and an industrial application. The numerical results show that the union methods achieve highly accurate solutions, while the fully immersed approach struggles with discontinuities in field gradients across material interfaces. Nevertheless, these methods significantly reduce the geometric preprocessing effort compared to conventional, conformal multi-patch analysis and require substantially fewer patches. Overall, this demonstrates that our immersed boundary-conformal isogeometric framework possesses great potential for efficient simulation of complex electromagnetic devices.

==> doc/makefile <==
# $Id: makefile 282 2026-01-08 05:54:22Z rishi $

file=elsdoc


all: pdf out 
	make pdf
	make pdf

#out:
#	if  [ -f $(file).out ] ; then cp $(file).out tmp.out; fi ;
#	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ;

out:
	if  [ -f "$(file).out" ] ; then cp "$(file).out" tmp.out; fi ; 
	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ; 
	sed -i 's/{\\376\\377/{/g' tmp.out ; 
	sed -i '/dtxmark/s/\\000//g' tmp.out
	sed -i 's/\\040/ /g' tmp.out ; 
	sed -i 's/\t/ /g' tmp.out

pdf:
	pdflatex $(file).tex

index:
	makeindex -s gind.ist -o $(file).ind $(file).idx 

changes:
	makeindex -s gglo.ist -o $(file).gls $(file).glo

xview:
#	xpdf -z 200 $(file).pdf &>/dev/null
	open -a 'Skim.app' $(file).pdf 

view:
	open -a 'Adobe Reader.app' $(file).pdf

ins:
	latex $(file).ins 

diff:
	diff $(file).sty ../$(file).sty |less

copy:
	cp $(file).sty ../



==> sections/FEM.tex <==
\section{Mapping}

In classical finite element method (FEM) we define our basis functions in the parent/reference domain and map it back to the physical domain. We can express this in mathematical writing by saying, $F : \hat{\Omega} \to \Omega$ where $\hat{\Omega}$ is the reference domain and $\Omega$ is the physical domain. Also $\tbx = F(\boldsymbol{\xi})$ where $\boldsymbol{\xi} = (\xi, \eta)$. Any surface in the physical domain can be parametrized/describe our physical domain or geometry by $F : \hat{\Omega} \to \Omega$ where $\hat{\Omega}$ with linear combination of n Lagrangian basis function $N_i(\xi,\eta)$ with the element nodal points $\tbX_i \in \bbR^2$
\begin{equation}
    F = (x(\xi,\eta),y(\xi,\eta))
\end{equation}
\begin{equation}
    \tbX^{h} =\displaystyle \sum_{i=1}^{n} N_i(\boldsymbol{\xi})\,\tbX_i
\end{equation}

the Jacobian which is the Jacobian of the geometric parametrization is defined as follows:
\begin{equation}
    \tbJ =: \nabla_{\boldsymbol{\xi}}\,\tbX^{h}(\boldsymbol{\xi})
\end{equation}

the physical coordinate approximation can be written as $\tbX^{h} = X^{h}_i\, e_i$ and the nabla operator $\nabla_{\boldsymbol{\xi}} = \frac{\partial}{\partial\xi_j} \, e_j$, hence the Jacobian can be expressed as:

\begin{equation}
    \tbJ =: \frac{\partial \tbX_i^{h}}{\partial \xi_j} e_i \otimes e_j
\end{equation}

which can then be expressed in two-dimensions with a matrix form in:
\begin{equation}
    \tbJ =: \begin{bmatrix}
        \frac{\partial \tbX_1}{\partial \xi_1} & \frac{\partial \tbX_1}{\partial \xi_2}\\[4mm]
        \frac{\partial \tbX_2}{\partial \xi_1} & \frac{\partial \tbX_2}{\partial \xi_2}
    \end{bmatrix} =:
    \begin{bmatrix}
        \frac{\partial x}{\partial \xi} & \frac{\partial x}{\partial \eta}\\[4mm]
        \frac{\partial y}{\partial \xi} & \frac{\partial y}{\partial \eta}
    \end{bmatrix}
\end{equation}

so we can see that the Jacobian is mainly dependent on the geometry parametrization.

In case we would like to get the derivatives of the shape functions in the physical domain:

\begin{equation}
    \frac{\partial N_i}{\partial \tbX} = \frac{\partial N_i}{\partial \boldsymbol{\xi}}\, \frac{\partial \boldsymbol{\xi}}{\partial \tbX}
\end{equation}

which is analogous to 

\begin{equation}
    \nabla_{\tbX} N(\boldsymbol{\xi}) = \nabla_{\boldsymbol{\xi}} N(\boldsymbol{\xi})\cdot \left(\nabla_{\boldsymbol{\xi}} \tbX^{h}(\boldsymbol{\xi}) \right)^{-1}
\end{equation}

this means that you can use any basis function to approximate the solution variables $u^h$ and there is no need to use an isoparametric element.

\begin{equation}
    \begin{bmatrix}
        \frac{\partial Ni}{\partial x}\\[3mm]
        \frac{\partial N_i}{\partial y}
    \end{bmatrix} =
    \begin{bmatrix}
        \xi_{,x} & \eta_{,x} \\[3mm]
        \xi_{,y} & \eta_{,y}
    \end{bmatrix}\, \begin{bmatrix}
        \frac{\partial N_i}{\partial \xi}\\[3mm]
        \frac{\partial N_i}{\partial \eta}
    \end{bmatrix}
\end{equation}

Furthermore if we want to get the inverse of the Jacobian defined above, we get the following

\begin{equation}
    \tbJ^{-1} = \begin{bmatrix}
        \frac{\partial x}{\partial \xi} & \frac{\partial x}{\partial \eta}\\[3mm]
        \frac{\partial y}{\partial \xi} & \frac{\partial y}{\partial \eta}
    \end{bmatrix}^{-1} = \frac{1}{\mathrm{det} \,\tbJ}\begin{bmatrix}
        \frac{\partial y}{\partial \eta} & -\frac{\partial x}{\partial \eta}\\[3mm]
        \frac{\partial y}{\partial \xi} & \frac{\partial x}{\partial \xi}
    \end{bmatrix}
\end{equation}

Hence if someone defined the Jacobian as the above, then the transformation for the gradients should be as follows:
\begin{equation}
    \nabla_{\tbX} N_i(\boldsymbol{\xi}) = \left(\tbJ^{-T}\right) \nabla_{\boldsymbol{\xi}} N_i(\boldsymbol{\xi})
\end{equation}

for the two-dimensional case the Jacobian $\tbJ^{-T} \in \bbR^{2\times2}$ while in the three-dimensional case $\tbJ^{-T} \in \bbR^{3\times3}$.

\subsection{How to judge the accuracy of my numerical solution?}
Suppose that we solved the 2D Laplace problem with the finite element method, so we have an approximate solution $\bu_h(x)$, and if we have the exact solution $\bu(x)$ of the PDE, then we can calculate multiple error estimation measures. We define the error of the solution as 
\begin{equation}
    e(\bx) = \bu(\bx) - \bu_h(\bx).
\end{equation}

\subsubsection{The $L^2$ norm error}
Our first error measure is the $L_{2}$ norm error, which is the root-mean-square error in our domain. It is a measure of how big is the difference between the finite element solution and the exact solution (if available).

\begin{equation}
    \label{eq: L2error}
    \| e \|_{L^2} = \left( \int_{\Omega} e^2(\bx)\, \rmd \Omega \right)^{1/2}
\end{equation}

This error is calculated by evaluating the approximate solution $\bu_h(x)$ and the exact solution $\bu(x)$ at each integration point $\bx$, where $\bx = (x,y)$. Given a computational domain $\Omega$, we discretize it into the $n_e$ number of finite elements $\Omega_e$, hence we can rewrite \cref{eq: L2error} as follows:
\begin{equation}
    \| e \|_{L^2} =\left(  \displaystyle \sum_{i=1}^{n} \int_{\Omega_e} \left(\bu(\bx) - \bu_h(\bx)\right)^2\, \rmd \Omega^e \right)^{1/2} 
\end{equation}
We map our integral to the parent element $\hat{\Omega^e}$ for each element:
\begin{equation}
    \| e \|_{L^2}^2 =  \displaystyle \sum_{i=1}^{n_e} \int_{\hat{\Omega}^e} \left(\bu(\boldsymbol{\xi}) - \bu_h(\boldsymbol{\xi})\right)^2\, \mathrm{det}(\tbJ(\boldsymbol{\xi}))\, \rmd \hat{\Omega}^e 
\end{equation}
We integrate using the Gaussian quadrature integration scheme:
\begin{equation}
    \| e \|_{L^2}^2 \approx  \displaystyle \sum_{i=1}^{n_e} \sum_{r=1}^{n_{qp}} \left(\bu(\boldsymbol{\xi}_r^e) - \bu_h(\boldsymbol{\xi}_r^e)\right)^2\,w^e_r\, \mathrm{det}(\tbJ(\boldsymbol{\xi}_r^e))\ 
\end{equation}

\subsubsection{The $L^\infty$ norm error}
The second error measure is the $L^\infty$ error, which represents the maximum error between the approximate solution and the exact solution, in other words, it shows the local accuracy of the approximate solution.

\begin{equation}
    \| e \|_{L^\infty}^2 = \mathrm{max}\, \left| e(\bx) \right|
\end{equation}


\subsubsection{The $H^1$ norm and seminorm}

The $H^1$ norm measures the difference in the solution and the gradients of the solution. In elasticity problems, it measures the difference in the displacement and the strains. 
\begin{equation}
    \| e \|_{H^1}^2 = \int_{\Omega} \left( e^2(\bx) + \left| \nabla e(\bx) \right|^2 \right) \rmd \Omega
\end{equation}

For the gradients part of the integral, we can compute it as follows:
\begin{equation}
     \left| \nabla e(\bx) \right|^2 = (\nabla e(\bx))^{\top} (\nabla e(\bx)) 
\end{equation}

where the gradients of the error is expanded as follows:
\begin{equation}
    \nabla e(\bx) = \nabla (\bu(\bx) - \bu_h(\bx)) = \nabla \bu(\bx) - \nabla \bu_h(\bx)
\end{equation}

For a given vector $\bv$, where $\bv = (v_x, v_y)$, the norm of the vector $v$ and the norm of its gradients $\nabla \bv$ can be calculated as follows:
\begin{equation}
    \left| \bv \right| = \sqrt{v_x^2 + v_y^2}
\end{equation}

\begin{equation}
    \nabla \bv = \begin{bmatrix}
        v_{x,x} & v_{x,y}\\
        v_{y,x} & v_{y,y}
    \end{bmatrix}
\end{equation}

and then the norm of the gradient is 

\begin{equation}
    \left| \nabla \bv \right| = v_{x,x}^2 + v_{x,y}^2 + v_{y,x}^2 + v_{y,y}^2
\end{equation}

%%%

\subsection{Assessing the accuracy of a numerical solution}

Assume that the 2D Laplace equation is solved using the finite element method, producing an approximate solution $\bu_h(x)$. If the exact solution $\bu(x)$ is also available, several quantitative error measures can be computed. We define the pointwise error as
\begin{equation}
    e(\bx) = \bu(\bx) - \bu_h(\bx).
\end{equation}

\subsubsection{The $L^2$ norm error}

The first error metric is the $L^2$ norm, which corresponds to the root-mean-square error over the domain. This norm provides a global measure of the magnitude of the deviation between the approximate and exact solutions.

\begin{equation}
    \label{eq: L2error}
    \| e \|_{L^2} = \left( \int_{\Omega} e^2(\bx)\, \rmd \Omega \right)^{1/2}
\end{equation}

To compute this error, both $\bu_h(x)$ and $\bu(x)$ are evaluated at each integration point $\bx = (x,y)$. For a discretized computational domain $\Omega$ consisting of $n_e$ finite elements $\Omega_e$, the expression in \cref{eq: L2error} becomes
\begin{equation}
    \| e \|_{L^2} =\left(  \displaystyle \sum_{i=1}^{n} \int_{\Omega_e} \left(\bu(\bx) - \bu_h(\bx)\right)^2\, \rmd \Omega^e \right)^{1/2}. 
\end{equation}

Mapping each element integral to its parent element $\hat{\Omega^e}$ yields
\begin{equation}
    \| e \|_{L^2}^2 =  \displaystyle \sum_{i=1}^{n_e} \int_{\hat{\Omega}^e} \left(\bu(\boldsymbol{\xi}) - \bu_h(\boldsymbol{\xi})\right)^2\, \mathrm{det}(\tbJ(\boldsymbol{\xi}))\, \rmd \hat{\Omega}^e .
\end{equation}

Using Gaussian quadrature, the error norm is approximated as
\begin{equation}
    \| e \|_{L^2}^2 \approx  \displaystyle \sum_{i=1}^{n_e} \sum_{r=1}^{n_{qp}} \left(\bu(\boldsymbol{\xi}_r^e) - \bu_h(\boldsymbol{\xi}_r^e)\right)^2\,w^e_r\, \mathrm{det}(\tbJ(\boldsymbol{\xi}_r^e))\ .
\end{equation}

\subsubsection{The $L^\infty$ norm error}

The second error metric is the $L^\infty$ norm, which captures the maximum pointwise error over the domain. This measure reflects the local accuracy of the numerical approximation.

\begin{equation}
    \| e \|_{L^\infty}^2 = \mathrm{max}\, \left| e(\bx) \right|
\end{equation}

\subsubsection{The $H^1$ norm and seminorm}

The $H^1$ norm accounts for differences not only in the solution values but also in their gradients. In elasticity, for example, this norm reflects discrepancies in both displacements and strains.

\begin{equation}
    \| e \|_{H^1}^2 = \int_{\Omega} \left( e^2(\bx) + \left| \nabla e(\bx) \right|^2 \right) \rmd \Omega
\end{equation}

The gradient contribution is computed as
\begin{equation}
     \left| \nabla e(\bx) \right|^2 = (\nabla e(\bx))^{\top} (\nabla e(\bx)).
\end{equation}

Since
\begin{equation}
    \nabla e(\bx) = \nabla (\bu(\bx) - \bu_h(\bx)) = \nabla \bu(\bx) - \nabla \bu_h(\bx),
\end{equation}
the gradient error can be evaluated directly if derivatives of both solutions are available.

For a vector field $\bv = (v_x, v_y)$, the vector norm and the Frobenius norm of its gradient are given by
\begin{equation}
    \left| \bv \right| = \sqrt{v_x^2 + v_y^2},
\end{equation}

\begin{equation}
    \nabla \bv = \begin{bmatrix}
        v_{x,x} & v_{x,y}\\
        v_{y,x} & v_{y,y}
    \end{bmatrix},
\end{equation}

from which the gradient norm is computed as
\begin{equation}
    \left| \nabla \bv \right| = v_{x,x}^2 + v_{x,y}^2 + v_{y,x}^2 + v_{y,y}^2.
\end{equation}

